Video Probabilistic Diffusion Models in Projected Latent Space

Despite the remarkable progress in deep generative models, synthesizing high-resolution and temporally coherent videos still remains a challenge due to their high-dimensionality and complex temporal dynamics along with large spatial variations. Recent works on diffusion models have shown their potential to solve this challenge, yet they suffer from severe computation- and memory-inefficiency that limit the scalability. To handle this issue, we propose a novel generative model for videos, coined projected latent video diffusion models (PVDM), a probabilistic diffusion model which learns a video distribution in a low-dimensional latent space and thus can be efficiently trained with high-resolution videos under limited resources. Specifically, PVDM is composed of two components: (a) an autoencoder that projects a given video as 2D-shaped latent vectors that factorize the complex cubic structure of video pixels and (b) a diffusion model architecture specialized for our new factorized latent space and the training/sampling procedure to synthesize videos of arbitrary length with a single model. Experiments on popular video generation datasets demonstrate the superiority of PVDM compared with previous video synthesis methods; e.g., PVDM obtains the FVD score of 639.7 on the UCF-101 long video (128 frames) generation benchmark, which improves 1773.4 of the prior state-of-the-art.

==> resources/is_table.tex <==
\begin{table}[ht!]
\caption{
IS values (higher values are better) of video generation models on UCF-101. Bolds indicate the best results and subscripts denote the standard deviations. We mark the method with * if the model is trained on the entire train+test split, otherwise the method uses only the train split for training.
}\label{tab:is} 
\centering\small
\begin{tabular}{lc}
    \toprule
    % \multicolumn{3}{c}{Train split} \\
    % \midrule
    Method & IS ($\uparrow$) \\
    \midrule
    VGAN~\citep{vondrick2016generating} & \phantom{0}8.31\stdv{0.09} \\
    TGAN~\citep{saito2017temporal}      & 11.85\stdv{0.07}  \\
    MoCoGAN~\citep{tulyakov2018mocogan} & 12.42\stdv{0.07}  \\
    ProgressiveVGAN~\citep{acharya2018towards} & 14.56\stdv{0.05}  \\
    LDVD-GAN~\citep{kahembwe2020lower}  & 22.91\stdv{0.19}  \\
    VideoGPT~\citep{yan2021videogpt}    & 24.69\stdv{0.30}  \\
    TGANv2~\citep{saito2020train}       & 28.87\stdv{0.67}  \\
    StyleGAN-V*~\citep{skorokhodov2021stylegan} & 23.94\stdv{0.73} \\ 
    DIGAN~\citep{yu2022digan}           & 29.71\stdv{0.53}  \\
    VDM*~\citep{ho2022video}            & 57.00\stdv{0.62}  \\
    TATS~\citep{ge2022long}             & 57.63\stdv{0.24}  \\
    \midrule
    \rowcolor{aliceblue}
    \sname (ours)   &  \textbf{74.40\stdv{1.25}} \\
    \bottomrule
\end{tabular}
\vspace{-0.1in}
\end{table}

